Framed Polytopes and Higher Categories

In the early 1990s, Kapranov and Voevodsky proposed a geometric method for constructing higher-categorical pasting diagrams from generically framed convex polytopes. This work revisits their construction and identifies a convex-geometric condition that is both necessary and sufficient for the procedure to yield a well-defined pasting diagram. Our criterion, the absence of cellular loops, relates their construction to the theory of cellular strings, an active area of convex geometry originating in the Baues problem. This paper introduces higher-dimensional cellular strings and uses them to disprove the Kapranov-Voevodsky conjecture in the following strong sense. Not only do we exhibit framed polytopes admitting cellular loops, but we also construct examples for which every admissible frame produces one. As observed by these authors, Street's orientals arise from canonically framed cyclic simplices. We establish that this family is exceptional as any random $n$-simplex, canonically framed, almost surely exhibits cellular loops in the large $n$-limit.

==> fig/street.tex <==
\begin{small}
	\begin{verbatim}
		[0,] | [1,]
		[0,1]
		---------------
		[0,] | [2,]
		[0,2] | [0,1] + [1,2]
		[0,1,2]
		---------------
		[0,] | [3,]
		[0,3] | [0,1] + [1,2] + [2,3]
		[0,2,3] + [0,1,2] | [0,1,3] + [1,2,3]
		[0,1,2,3]
		---------------
		[0,] | [4,]
		[0,4] | [0,1] + [1,2] + [2,3] + [3,4]
		[0,3,4] + [0,2,3] + [0,1,2] | [0,1,4] + [1,2,4] + [2,3,4]
		[0,2,3,4] + [0,1,2,4] | [0,1,2,3] + [0,1,3,4] + [1,2,3,4]
		[0,1,2,3,4]
	\end{verbatim}
\end{small}

==> sec/counterexamples.tex <==
% !TEX root = ../polycat.tex

\subsection{Framed polytopes and systems of projections}\label{s:counterexamples}

%As reviewed in \cref{s:conjectures}, Kapranov and Voevodsky considered Johnson's model of pasting diagrams when introducing their conjecture.
%After this conjecture was stated, and presumably influenced by its chain complex language, Steiner introduced the model reviewed in \cref{s:steiner}, which does does not suffer from the limitations identified by Forest in Johnson's approach \cite{forest2022pasting}.
Since the previous theorem provides necessary and sufficient conditions for a framed polytope to define a Steiner diagram---namely, the absence of cellular loops---it remains to establish the equivalence between our framed polytope language and the system of projections language used by Kapranov and Voevodsky.

%We will use it to provide necessary and sufficient conditions for the Kapranov--Voevodsky conjecture to hold after showing the
%We remark that our counterexamples can be shown to disprove the conjecture and its weak form in any existing formalization of pasting diagrams since every one of them rules out the presence of loops.

%Let us express the Kapranov--Voevodsky conjecture and its weak version in terms of framed polytopes instead of admissible systems of projections.
%Please recall from \cref{s:conjectures} the poset orientation $\gamma(p)$ on $\nefaces$ constructed from an admissible system of projections $p$.

\medskip\lemma The system of projections of a framed polytope is admissible and its induced \(f\)-orientation agrees with the one constructed by Kapranov--Voevodsky.
Furthermore, for any admissible system of projections on a polytope \(P\) there is a $P$-admissible frame inducing the same \(f\)-orientation.

\begin{proof}
	Recall the Kapranov--Voevodsky construction from \cref{s:conjectures}.
	The admissibility of the system of projections of a $P$-admissible frame follows directly from the definition of $P$-admissibility.
	We need to show that the source of an arbitrary face $F$ with respect to the $f$-orientation $\beta$ induced by the given frame agrees with the source of $F$ defined by the Kapranov--Voevodsky \(f\)-orientation $\gamma$.
	According to \cref{lem:projectiondescription}, the $\beta$ source of the $k$-face $F$ consists of all $E \lessdot F$ such that
	\[
	\sprod{\normal_{\pi_k E}^{\pi_k F}}{v_k} < 0.
	\]
	The $\gamma$ source of $F$ consists of all $E \lessdot F$ for which there exists an affine-linear function $u(w)$ which is $0$ on $p_k(E)$ and non-negative on $p_k(F)$ such that $u(w) \to \infty$ as $w \to \infty$ in the oriented fiber of $\pi_{k-1}^k$.
	The fiber of the projection $\pi_{k-1}^k$ is generated and oriented by $v_k$.
	The choice
	\[
	u(w) \defeq \max_{x \in P}\sprod{\normal_{\pi_k E}^{\pi_k F}}{x} - \sprod{\normal_{\pi_k E}^{\pi_k F}}{w}
	\]
	shows the agreement of both \(f\)-orientations.

	For the last claim, consider a \(P\)-admissible system of projections $p$
	\[
	\R \xla{p_1^2} \R^2 \xla{p_2^3} \dotsb \xla{p_{n-2}^{n-1}} \R^{n-1} \xla{p_{n-1}^n} \R^n.
	\]
	Let $v_1$ be the canonical generator of $\R$.
	Let us assume for an induction argument that $(v_1,\dots,v_k)$ have been chosen so that $\Span(v_1,\dots,v_j) = \R^j$ as oriented vector spaces and $p_j^{j+1} = \pi_j^{j+1}$ for any $1 \leq j < k$.
	Choose an oriented generator of $\ker p_k^{k+1}$ and define it to be $v_{k+1}$.
	We have $\Span(v_1,\dots,v_{k+1}) = \R^{n+1}$ as oriented vector spaces and $p_k^{k+1} = \pi_k^{k+1}$, as claimed.
\end{proof}

%Using this lemma, the Kapranov--Voevodsky conjecture can be formalized as stating that \textit{the chain complex of any framed polytope is a Steiner diagram.}
%By \cref{t:loop-free}, this is equivalent to the claim that every framed polytope has no cellular loops.
%A claim falsified by the many examples constructed in \cref{part:strings}.
%Similarly, the weak version of this conjecture: \textit{For any polytope \(P\) there is a \(P\)-admissible frame with respect to which its chain complex is a Steiner diagram} is falsified by
%is equivalent to the following: \textit{Given a polytope $P$, there is a $P$-admissible frame making it into a framed polytope whose chain complex is a Steiner diagram.}
%By \cref{t:loop-free} again, this is equivalent to the existence of a $P$-admissible frame making $P$ into a framed polytope with no cellular loops for any polytope $P$.
%A claim falsified by
%the example constructed in \cref{s:loop-inevitability}.
%As mentioned in \ref{ss:diagrams}, all formalizations of pasting diagrams preclude the existence of directed loops, which makes our counterexamples model-independent.



==> sec/fiber.tex <==
% !TEX root = ../polycat.tex

\subsection{Fiber polytopes}\label{s:fiber}

Together with the original reference \cite{BilleraSturmfels1992}, we cite \cite[Lec.~9]{Ziegler95} and \cite[Sec.~9.1]{deloeraTriangulations2010} for a thorough exposition of fiber polytopes.

%\SS Let $\pi \colon P \to Q$ be a projection of polytopes with $P \subset \R^p$ and $Q \subset \R^q$.
%From \cref{s:subdivision}, recall the notions of $\pi$-induced and $\pi$-coherent subdivision.
%We define a partial order on $\pi$-induced subdivisions by declaring \(\cS_1 \leq \cS_2\) if and only if the union of the polytopes in \(\cS_1\) is contained in the union of the polytopes in \(\cS_2\) or, more subcintly, if $\bigcup \cS_1 \subseteq \bigcup \cS_2$.
%The poset of \(\pi\)-coherent subdivisions, with the induced order, will be denoted $\omega_\pi$.

\SS Let $\pi \colon P \subset \R^p \to Q \subset \R^q$ be a projection of polytopes.
%$P \subset \mathbb{R}^p$ and $Q \subset \mathbb{R}^q$.
From \cref{s:subdivision}, recall the notions of $\pi$-induced and $\pi$-coherent subdivisions.
We define a partial order on $\pi$-induced subdivisions by declaring $\mathcal{S}_1 \leq \mathcal{S}_2$ if and only if the union of the polytopes in $\mathcal{S}_1$ is contained in the union of the polytopes in $\mathcal{S}_2$.
More succinctly, $\mathcal{S}_1 \leq \mathcal{S}_2$ if $\bigcup \mathcal{S}_1 \subseteq \bigcup \mathcal{S}_2$.
The poset of $\pi$-coherent subdivisions, with the induced order, will be denoted $\omega_\pi$.

\SS Following \cite{BilleraSturmfels1992}, the subset of $\R^p$ defined by 
\[
\fiber_\pi = \frac{1}{\mathrm{vol}(Q)} \int_Q \pi^{-1}(x) \, dx
\]
is a polytope of dimension $\dim(P) - \dim(Q)$ contained in the intersection of $P$ and the preimage of the barycenter $\int_Q x \, dx$ of $Q$.
$\fiber_\pi$ is referred to as the \defn{fiber polytope} of $\pi$.

The posets $\hat\cL(\fiber_\pi)$ and $\omega_\pi$ can be identified with each other.
Explicitly, to a face $\fiber_\pi^\psi$ -- where $\psi \in (\R^p)^*$-- we assign the only $\pi$-coherent subdivision $\cS^\psi$ satisfying
\[
\textstyle\bigcup\cS^\psi = \set{\pi^{-1}(x)^{\psi} \mid x \in Q}.
\]
Conversely, to a $\pi$-coherent subdivision with functional $\psi \in (\R^p)^*$ we assign the face $\fiber_\pi^\psi$ explicitly described by
\[
\frac{1}{\mathrm{vol}(Q)} \int_Q \pi^{-1}(x)^\psi \, dx.
\]

%Given $G \in \hat\cL(\Sigma_\pi)$, we denote its associated \(\pi\)-coherent subdivision by $\cF^G$, and the subset of top-dimensional elements in $\cF^G$ by $\mathring\cF^G$.

\SS Let $E$ be a face of $Q$.
Denote $P \cap \pi^{-1}(Q)$ by $P_E$ and the restriction of $\pi$ to it by $\pi_E$.
Any $\pi$-induced subdivision $\cS$ determines a $\pi_E$-induced one given by $\cS_E \defeq \set{F \cap P_E \mid F \in \cS}$.
Furthermore, if $\cS$ is $\pi$-coherent then $\cS_E$ is $\pi_E$-coherent with respect to the same functional.
\anibal{I think that there must be an affine projection $\fiber_\pi \to \fiber_{\pi_E}$ inducing this lattice map. Is that so?}


%--------
%
%Naturally, a $\pi$-induced subdivision of $Q$ can be restricted to any of its faces.
%Explicitly, for a face $E$ of $Q$ the \defn{restriction} of $\cF$ to $E$ is defined by $\cF_E \defeq \set{\pi^{-1}(E) \cap F \mid F \in \cF}$.


%Explicitly, the isomorphism is given by
%\[
%\begin{tikzcd}[column sep=small, row sep=0]
%	\hat\cL(D_P) \rar["\cong\ "] & \omega^\alpha_{\text{coh}}(P) \\
%	G \rar[mapsto] & \overline\fB_G,
%\end{tikzcd}
%\]


%We define a partial order on these subdivisions by setting \(\cF_1 \leq \cF_2\) if and only if the union of the polytopes in \(\cF_1\) is contained in the union of the polytopes in \(\cF_2\). This means that the subdivision \(\{\pi(F) : F \in \cF_1\}\) of \(Q\) is a refinement of the subdivision induced by \(\cF_2\).
%
%The resulting partially ordered set, containing all subdivisions of \(Q\) that are induced by \(\pi : P \rightarrow Q\), will be denoted by \(\omega(P,Q)\).
%
%For example, consider the projection sketched before, and label the vertices and edges of \(P\):
%
%In this situation, there are three subdivisions of \(Q \cong \R\) induced by the projection from \(P \cong \R^2\), given by
%\[
%\cF_0 = \{V_1, P, E_3\},
%\]
%\[
%\cF_1 = \{V_1, E_1, V_2, E_2, V_3\},
%\]
%\[
%\cF_2 = \{V_1, E_5, V_5, E_4, V_4\}.
%\]
%
%Note that the actual tilings \(\pi(\cF_1)\), \(\pi(\cF_2)\) of \(Q\) coincide, but they are distinguished since they correspond to distinct collections \(\cF_1, \cF_2 \subseteq \mathcal{L}(P)\).
%
%Condition (ii) in Definition 9.1 excludes "noncontinuous" sections like \(\{V_1, E_1, V_2, E_4, V_4\}\). Thus, a \(\pi\)-induced subdivision of \(Q\) is given by a family \(\cF\) of faces of \(P\) - note that the projected set \(\{\pi(F) : F \in \cF\}\) is not sufficient to determine the subdivision as defined in Definition 9.1.
%
%Condition (ii) is stronger than just requiring that \(\pi(F) \cap \pi(F') \neq \emptyset\) implies \(F \subseteq F'\): for example, families like \(\{V_1, P, V_3\}\) are also excluded. Condition (ii) also implies that every collection \(\cF \subseteq \mathcal{L}(P)\) is completely determined by its inclusion-maximal members.
%
%The partial order that we get for our example is
%\[
%\cF_0 \rightarrow \cF_1 \leftrightarrow \cF_2,
%\]
%which corresponds to the nonempty faces of a 


==> sec/molecules.tex <==
% !TEX root = ../polycat.tex

\section{Shellings and molecules}\label{part:molecules}


Finally, we show that framed polytopes provide examples of regular directed complexes in the sense of \cite{Steiner93,Hadzihasanovic20}, using the line shellings of facets induced by the frame, and outline connections with the theory of higher-categorical diagrams being currently developed in~\cite{Hadzihasanovic24}.

Our goal in this section is to show (\cref{thm:gobular-structure}) that orientation structures associated to framed polytopes are regular directed complexes in the sense of \cite{Hadzihasanovic24,Hadzihasanovic20,Steiner93}.
To do so, we enlarge our definition of source and target to coherent subdivisions (\cref{def:Pk-admissible}) and we use the line shellings of facets induced by the frame (\cref{prop:shelling}).
The geometry of the situation has a very intuitive categorical meaning: line shellings give the order in which cells are composed via whiskering (\cref{cor:st-molecules}).
An interesting consequence is that the $k$-source and $k$-target of a framed polytope are always $(k-1)$-loop free~(\cref{rem:loop-freeness-source-target}).

\SS

Let $P$ be a polytope with a poset orientation.
The \defn{closure} of a subset $U \subset \faces$ is the set $\overline{U} : = \{ F \in \faces \ | \ \exists G \in U, F \subset G \}$ of all faces of faces in~$U$.
We say that $U$ is \defn{closed} if $\overline{U} = U$.

\SS \label{def:k-source-target-bis}

For~$k\geq 0$, the \defn{$k$-source}~$\so_k(U)$ (resp.\ \defn{$k$-target}~$\ta_k(U)$) of a closed subset~$U \subset \faces$ is the set of $k$-faces~$F$ in~$U$ such that every covering relation~$F \lessdot G$ with~$G$ in~$U$ has label~$-$ (resp.\ $+$).

\SS

\remark
In contrast to the preceding definition \cref{def:source-target}, according to \cref{def:k-source-target-bis} the $k$-source~$\so_k(\overline{F})$ or target~$\ta_k(\overline{F})$ of a $k$-face $F$ is defined, and equal to~$F$ itself.

\SS

The set of \defn{maximal elements} of a closed subset $U \subset \faces$ is
\[\max(U) \defeq \{F \in U \ | \ \forall \ G \in U, F \subset G \implies F = G\}.\]
We denote by $\max_{< k}(U)$ the subset of faces of $\max(U)$ of dimension~$<k$.

\SS \label{def:boundaries}

The \defn{$k$-input} and \defn{$k$-output boundaries} of a closed subset $U$ are defined by
\[
	\bso_k(U) \defeq \overline{\so_k(U)} \cup \overline{\max\nolimits_{< k}(U)}
	\quad \text{and} \quad
	\bta_k(U) \defeq \overline{\ta_k(U)} \cup \overline{\max\nolimits_{< k}(U)}.
\]
We denote by $\bso_k(F)\defeq \bso_k(\overline{F})$ (resp.\ $\bta_k(F) \defeq \bta_k(\overline{F})$) the $k$-input (resp.\ output) boundary of a face~$F \in \faces$.
Note that in this case, we have $\bso_k(F) = \overline{\so_k(F)}$ (resp.\ $\bta_k(F) = \overline{\ta_k(F)}$).

\SS

The \defn{dimension} of a subset $U \subset \faces$ is the maximum dimension of an element in $U$.
If $U$ is of dimension $n$, we abbreviate $\bso_{n-1}(U)$ and $\bta_{n-1}(U)$ by $\bso(U)$ and $\bta(U)$.

\SS \label{def:atoms-molecules}

An \defn{atom} consists of the closure $\overline{F}$ of a face $F \in \faces$.
For $U$ a closed subset of $\faces$, we say that $U$ is a \defn{molecule} if it is an atom, or if there exist molecules~$U_1,U_2 \subsetneq U$ and $k \in \N$ such that $U = U_1 \cup U_2$ and $U_1 \cap U_2 = \bta_k(U_1) = \bso_k(U_2)$.

\SS

A polytope $P$ with a poset orientation is a \defn{regular directed complex} if for all $d$-dimensional faces~$F \in \faces$, we have that
\begin{enumerate}
	\item \label{it:globularcond1} $\bso(F)$ and $\bta(F)$ are molecules,
	\item \label{it:globularcond2} $\bso(\bta(F)) = \bso(\bso(F))$ and $\bta(\bso(F)) = \bta(\bta(F))$ if $d>1$,
	\item \label{it:globularcond3} $\bso_k(F) \cap \bta_k(F) = \bso_{k-1}(F) \cup \bta_{k-1}(F)$ for all $k < d$.
\end{enumerate}
The identities~\eqref{it:globularcond2} are called the \defn{globular identities}.

\SS

\remark
We use here the definition of regular directed complex from~\cite[Def.~1.29]{Hadzihasanovic20}.
Little work shows that it is equivalent to~\cite[Def.~5.3.1]{Hadzihasanovic24}.

\SS

Our goal is to prove in \cref{thm:gobular-structure} that framed polytopes are regular directed complexes.
Conditions \eqref{it:globularcond2} and \eqref{it:globularcond3} above are easy to verify.
To prove that sources and targets are molecules, we will slightly enlarge our setup: we generalize the definition of input and output boundaries, and prove the stronger statement that these satisfy \eqref{it:globularcond1}.

\SS \label{def:new-sources-and-targets}

Let~$P$ be a polytope in $\R^d$ and let~$B$ be a frame of~$\R^d$ which is \emph{not necessarily $P$-admissible}. Let $F\in\faces$ be a face of dimension $\dim F>k$ such that $\dim(\pi_{k+1}(F)) = k+1$.
The \defn{$k$-source}~$\so_k(F)$ (resp. \defn{$k$-target}~$\ta_k(F)$) of~$F$ is the set of faces~$\pi_{k+1}^{-1}(G)\cap F$ where~$G$ is a facet of~$\pi_{k+1}(F)$ such that
\[
\sprod{\normal_{G}^{\pi_{k+1} F}}{v_{k+1}} < 0 \quad (\text{resp.} > 0).
\]
For $P$-admissible frames, this coincides with the definitions given in~\cref{lem:projectiondescription}.
Note that if the frame is not admissible, then the $k$-source and $k$-target can contain faces of dimension larger than~$k$.

\SS

For a closed subset~$U \subset \faces$, $\so_k(U)$ (resp. $\ta_k(U)$)
is the subset of faces $F\in U$ such that $\dim(\pi_{k+1}(F)) = k$ but that do not belong to any $\ta_k(F)$ (resp. $\so_k(F)$) for an $F\in U$ such that $\dim(\pi_{k+1}(F)) = k+1$. We define $\max_{< k}(U)$ as the set of faces of $\max(U)$ such that the projection $\pi_{k+1}$ is of dimension smaller than~$k$.
We then define \defn{$k$-input} and \defn{$k$-output boundaries}, \defn{atoms} and \defn{molecules} exactly as in~\cref{def:boundaries} and~\cref{def:atoms-molecules}.
Again, note that for $P$-admissible frames, this coincides with the previous definitions.

\SS

\remark
Our definition of $k$-source and target is just a reformulation of the concept of \emph{$\pi_k$-induced coherent subdivision} of $\pi_{k}(F)$ as introduced in~\cite{BilleraSturmfels1992}, see also \cite[Def.~9.2]{Ziegler95}.
Comparing with \cref{s:subdivision}, the $k$-source and target are still coherent subdivisions of $\pi_k(F)$, but they are no longer necessarily tight.
Looking back at \cref{thm:globular-flag-chirotopes}, under this new definition we have that orientation structures of framed simplices are in bijection with acyclic realizable full flag chirotopes, which are no longer necessarily uniform.

\SS

Some non-admissible frames will appear naturally in our proofs.
However, to simplify the exposition, it is simpler if we do concentrate on frames that have only certain degeneracies.

\SS \label{def:Pk-admissible}

Let $P \subset \R^d$ be a polytope.
We say that a frame $(v_1,\dots,v_d)$ is \defn{$P_k$-admissible} if $(v_1,\dots,v_k)$ is {$\pi_k(P)$-admissible}.
That is, all possible degeneracies arise from the first projections, but the vectors $v_1,\dots,v_k$ can be perturbed without altering the orientation structure of~$P$.

\SS \label{def:shelling}

Let $P$ be a full-dimensional polytope in $\R^d$ and $B = (v_1,\ldots,v_d)$ be a $P_k$-admissible frame for some $1<k<d$.
Define the vector $${w_{k+1}(\lambda)} \defeq \lambda v_{k+1}-v_{k}$$ depending on a parameter~$\lambda \in \R$.
For each facet~$F_i$ of $\pi_{k+1}(P)$, define $\lambda_i$ as the value for which $\sprod{\normal_{F_i}}{w_{k+1}(\lambda_i)} = 0$.
That is, we define $$\lambda_i \defeq \frac{\sprod{\normal_{F_i}}{v_{k}}}{\sprod{\normal_{F_i}}{v_{k+1}}}.$$
To avoid degeneracy problems when two $\lambda_i$'s coincide, we consider a small perturbation $v_{k}'$ of $v_{k}$ and set
$\lambda_i' \defeq \frac{\sprod{\normal_{F_i}}{v_{k}'}}{\sprod{\normal_{F_i}}{v_{k+1}}}$.
We require the perturbation to be small enough so that it does not change the order of any two different $\lambda_i$'s, and generic enough so that $\lambda_i'\neq \lambda_j'$ for $i\neq j$.
Note that, since the frame is $P_k$-admissible, this does not alter the orientation structure of~$P$.

\SS

We then define total orders $<_{\so}$ and $<_{\ta}$ of the faces in $\so_k(P)$ and $\ta_k(P)$.
Each element $G_i\in\so_k(P)$ or $G_i\in\ta_k(P)$ is of the form~$\pi_{k+1}^{-1}(F_i)\cap P$ for a facet~$F_i$ of~$\pi_{k+1}(P)$.
We set $G_i<_{\so} G_j$ if $\lambda_i'>\lambda_j'$ for $G_i,G_j\in \so_k(P)$, and $G_i<_{\ta} G_j$ if $\lambda_i'<\lambda_j'$ for $G_i,G_j\in \ta_k(P)$.

\SS

For admissible frames, these orderings give rise to \emph{line shellings} of the source and the target.
A \emph{shelling} of a CW-complex is a total ordering of the facets with some specific gluing properties.
For more details, see for example \cite[Sec.~8.1]{Ziegler95}.

\SS \label{prop:shelling}

\proposition
For any two faces $F_1,F_2$ in the $k$-source (resp.\ $k$-target) of a polytope $P$ with respect to a $P_k$-admissible frame,
if~$\ta_{k-1}(F_1)\cap \so_{k-1}(F_2)\neq \emptyset$ then we have $F_1 <_{\so} F_2$ (resp. $F_1 <_{\ta} F_2$).

\begin{proof}
We do the proof for the target, and the proof for the source is analogous.
Note that if a face $F_i$ belongs to the $k$-target of~$P$ then $G_i \defeq \pi_{k+1}(F_i)$ is a facet of $\pi_{k+1}(P)$ whose outer normal vector has positive scalar product with $v_{k+1}$ (\cref{def:new-sources-and-targets}).
We can thus choose an outer normal vector $\normal_i$ such that $\sprod{\normal_i}{v_{k+1}} = 1$.
Now let $G \defeq G_1\cap G_2$ be the $(k-1)$-face given by the intersection of the two facets.
We have that $\normal_2 - \normal_1$ is an outer normal vector of $\pi_{k}(G)$ with respect to $\pi_{k}(F_1)$ in~$V_{k}$.
Since $\ta_{k-1}(F_1)\cap \so_{k-1}(F_2)\neq \emptyset$, this means that $\sprod{\normal_2-\normal_1}{v_{k}}>0$.
Therefore, we have $\sprod{\normal_1}{v_{k}}<\sprod{\normal_2}{v_{k}}$.
Since $\sprod{\normal_i}{v_{k+1}} = 1$, this means that $\lambda_1<\lambda_2$ and that we have~$F_1 <_{\ta} F_2$.
\end{proof}

\SS \label{rem:loop-freeness-source-target}

\remark
This gives a proof of $(k-1)$-loop-freeness for the $k$-source and $k$-target of a framed polytope.
Indeed, since $<_{\so}$ and $<_{\ta}$ are total orders, there is no cellular $(k-1)$-strings of infinite length.
This generalizes \cref{prop:dimP-2}.

\SS\label{cor:st-molecules}
\theorem
Let $P\subset \R^d$ be a polytope, let $F$ be a face of~$P$, and let $k \leq \dim F$.
Let $B = (v_1,\ldots,v_d)$ be a $P_k$-admissible frame.
Then, the $k$-input and output boundaries~$\bso_k(F)$ and $\bta_k(F)$ are molecules.

\begin{proof}
	We loose no generality by assuming $F = P$.
	Moreover, it suffices to show the statement for $\bso_k(P)$, the case of $\bta_k(P)$ is similar.
	We will assume that the $\lambda_i$'s from~\cref{def:shelling} are all distinct, as otherwise we can replace $v_k$ by $v_k'$, as in~\cref{def:shelling}, without altering the orientation structure.
	We proceed by induction on~$k \geq 0$.
	For~$k = 0$, we have that $\bso_0(P)$ is always a face of $P$, thus an atom and a molecule.
	Suppose that the statement holds for any~$k'< k$, and let $P$ be a polytope of dimension $\dim P \geq k+1$.
	Let us show that~$\bso_{k}(P)$ is a molecule.

We consider the total order $G_1,\ldots,G_\ell$ on the maximal faces of~$\bso_{k}(P)$ from \cref{def:shelling}.
We now show by induction on $j \geq 0$ that $\cG_j \defeq \bso_{k-1}(P) \cup \bigcup_{i = 1}^{j} \overline{G_i}$ is a molecule.
For $j = \ell$, this will prove that $\bso_{k}(P)$ is a molecule, completing the induction step.
For $j = 0$, there is nothing to show, since $\bso_{k-1}(P)$ is a molecule by the induction hypothesis on $k$.
Suppose now that $\cG_j$ is a molecule for any $j \leq m$.
We want to show that $\cG_{m+1}$ is a molecule.
For this, it suffices to show that $\cH_{m+1} \defeq \overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule.
Indeed, by \cref{prop:shelling}, we have the inclusion~$\bso_{k-1}(G_{m+1}) \subset \bta_{k-1}(\cG_m)$, and thus~$\bta_{k-1}(\cG_m) = \bso_{k-1}(G_{m+1} \cup \bta_{k-1}(\cG_m))$.
Assuming that $\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule allows one to write $\cG_{m+1} = \cG_m \cup \overline{G_{m+1}}$ as a gluing of two molecules satisfying the recursive definition \cref{def:atoms-molecules}.
Therefore, we are left with showing that~$\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule.

To prove that~$\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule, we will show that it is precisely the $(k-1)$-output boundary of $P$ for the frame
\[\tilde B(\lambda_{m+1}) = (v_1,\dots,v_{k-1},\tilde v_k \defeq v_{k+1},\tilde v_{k+1} \defeq w_{k+1}(\lambda_{m+1}),v_{k+2},\ldots),\]
and conclude by induction.
To avoid confusion, we denote by $\tilde \pi_1,\ldots,\tilde \pi_n $ the system of projections associated to~$\tilde B$.
Our induction will prove that $\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule for~$\tilde B$.
However, note that $\pi_j = \tilde \pi_j$ for all~$j$ except for~$j = k$ and~$j = k+1$.
In particular, we have $\pi_{k-1} = \tilde \pi_{k-1}$.
As the first~$k-1$ vectors of both frames coincide, all $j$-sources and targets with $j < k-1$ coincide for both frames.
Therefore, proving that $\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule for~$\tilde B$ implies that is is a molecule for~$B$, which is the result that we need.

We start by describing recursively $\bta_{k-1}(\cG_m)$.
Its maximal faces are, by definition, those that are in the $(k-1)$-target of some face in $\cG_m$, but not in the $k-1$-source of any other face.
For~$m = 0$, we have $\cG_0 = \bso_{k-1}(P)$ and $\bta_{k-1}(\cG_0) = \cG_0 = \bso_{k-1}(P)$.
For $m\geq 0$, we have that $\bso_{k-1}(G_{m+1})$ is included in $\bta_{k-1}(\cG_{m})$.
Indeed, by~\cref{prop:shelling} any maximal face in $\bso_{k-1}(G_{m+1})$ belongs to either~$\bso_{k-1}(P)$ or to~$\bta_{k-1}(G_{i})$, for some face~$G_i$ with~$i<m$, which belongs to $\cG_m$ by definition.
These maximal faces of~$\bso_{k-1}(G_{m+1})$ do not belong to~$\bta_{k-1}(\cG_{m+1})$.
In contrast, the maximal faces of~$\bta_{k-1}(G_{m+1})$, which are in~$\bta_{k-1}(\cG_{m+1})$: by \cref{prop:shelling} again, they do not belong to any~$G_i$ with~$i<m$.
Thus, at the level of maximal faces, the output boundary~$\bta_{k-1}(\cG_{m+1})$ is the symmetric difference of $\bta_{k-1}(\cG_{m})$ with the $(k-1)$-boundary of~$G_{m+1}$, replacing its source by its target.

Let's see that the same recursive description holds for the $(k-1)$-output boundary of~$P$ with respect to the frame $\tilde B(\lambda)$ as $\lambda$ increases.
When $\lambda$ has a very large negative value, the direction of $w_{k+1}(\lambda)$ is very close to~$-v_{k+1}$, and thus $\tilde \pi_k(P)$ is very close to $\pi_k(P)$.
With a triangular transformation as in \cref{ss:lowertriangular}, we can add $\frac{1}{|{\lambda}|}\tilde v_{k+1} = - v_{k+1}-\frac{1}{|{\lambda}|}v_{k}$ to $\tilde v_k = v_{k+1}$ to obtain $- \frac{1}{|{\lambda}|}v_{k}$.
So, we see that the $(k-1)$-target (or equivalently its closure, the $(k-1)$-output boundary) of~$P$ with respect to~$\tilde B$ coincides with the $(k-1)$-source (or equivalently its closure, the $(k-1)$-input boundary) of $P$ with respect to~$B$.
Similarly, we can see that if $\lambda$ has very large positive value, then the $(k-1)$-target for $\tilde B$ coincides with the $(k-1)$-target for~$B$.
The only possible changes in the $(k-1)$-target of $\tilde B(\lambda)$ appear for~$\lambda = \lambda_i$.
For~$\lambda = \lambda_i-\varepsilon$, with $\varepsilon$ a small positive number, the source of~$G_i$ is in $(k-1)$-target of $\tilde B(\lambda)$.
For~$\lambda = \lambda_i$ the whole face~$G_i$ enters the $(k-1)$-target of~$\tilde B(\lambda)$, while for $\lambda = \lambda_i+\varepsilon$, only its target remains in the $(k-1)$-target of $\tilde B(\lambda)$.

Therefore, we have that~$\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is the $(k-1)$-output boundary of $P$ for the frame $\tilde B(\lambda_{m+1})$.
By the induction hypothesis on $k$, we have that~$\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ is a molecule, which finishes the proof.
\end{proof}

%\SS

%\remark
%An alternative, more direct way to recover the description of~$\overline{G_{m+1}} \cup \bta_{k-1}(\cG_m)$ in \cref{cor:st-molecules} is to directly describe the facets of $\tilde \pi_k(P)$.
%By \cite[Thm.~1.4]{Ziegler95}, the facets of $\tilde \pi_{k}(P)$ are the image of either a facet of $\pi_{k+1}(P)$ whose normal vector is orthogonal to $w_{k+1}(\lambda)$, or the image of the common $(k-1)$-face of two facets $\pi_{k+1}(P)$ whose normal vectors have opposite sign when scalarly multiplied with $w_{k+1}(\lambda)$ (and in this case the normal vector of the face of the projection is the positive combination of the two normal vectors that is orthogonal to $w_{k+1}(\lambda)$). By construction, there is only one facet whose normal is orthogonal to $w_{k+1}(\lambda_{m+1})$, namely $G_{m+1}$. `Upper' facets of $\pi_{k+1}(P)$ with respect to $w_{k+1}(\lambda)$ (in the sense that they have positive scalar product), are the $G_{i} \in \so_k(P)$ with $\lambda_i<\lambda_{m+1}$ and the $G_{j} \in \ta_k(P)$ with $\lambda_j>\lambda_{m+1}$. Analogously, 'lower' facets of $\pi_{k+1}(P)$ with respect to $w_{k+1}(\lambda)$ are the $G_{i} \in \so_k(P)$ with $\lambda_i>\lambda_{m+1}$ and the $G_{j} \in \ta_k(P)$ with $\lambda_j<\lambda_{m+1}$. This gives us the facets of $\tilde \pi_k(P)$. Looking a the sign of the scalar product of their normal vector with $v_{k+1}$ shows that the facets of $\tilde \pi_k(P)$ that are in the $(k-1)$-target for $\tilde B(\lambda_{m+1})$ are those in $G_{m+1} \cup \ta_{k-1}(\cG_m)$, as claimed. This concludes the proof.

\SS \label{thm:gobular-structure}

\theorem
Framed polytopes are regular directed complexes.

\begin{proof}
Let $(P,B)$ be a framed polytope with frame~$B = (v_1,v_2,\ldots)$, and let $F$ be a face of dimension $\dim F = d$.
We need to check the $3$ conditions from \cref{def:globular-structure}. % WRONG LABEL
Condition \eqref{it:globularcond1} is a special case of~\cref{cor:st-molecules}.
It suffices to prove Condition~\eqref{it:globularcond2} for the $k$-input boundary, the output case is similar.
From \cref{s:computing_sk_and_tk} and \cref{s:subdivision} we get directly $$\bso(\bso(F)) = \bso(\pi_{d-1}(\bso(F))) = \bso(\pi_{d-1}(F)) = \bso(\pi_{d-1}(\bta(F))) = \bso(\bta(F)),$$ as desired.
Alternatively, one can use \cref{p:oriented-thin} for a combinatorial, instead of geometric proof.
It remains to prove Condition~\eqref{it:globularcond3}.
From \cref{s:computing_sk_and_tk}, we know that $\bso_k(F)\cup \bta_k(F) = \overline{\bd^{(k)}(F)}$.
We thus need to show that $\bso_{k+1}(F)\cap \bta_{k+1}(F) = \overline{\bd^{(k)}(F)}$.
Since $\bso_k(F) = \bso(\pi_{k+1}(F))$ for any $k$, it suffices to show that $\bso(F) \cap \bta(F) = \overline{\bd^{(d-2)}(F)}$, and the result follows by induction.
Returning to the definition \cref{def:boundary}, the maximal faces of $\overline{\bd^{(d-2)}(F)}$ are the facets of $\pi_{d-1}(F)$.
Since the frame~$B$ is~$P$-admissible, these are precisely the $(d-2)$-faces of $F$ which are the intersection $G \cap G'$ of two facets~$G,G'$ of~$F$ with $\sprod{\normal_G}{v_{d}}\sprod{\normal_{G'}}{v_{d}}<0$.
According to~\cref{lem:projectiondescription}, these are exactly the maximal faces of the intersection~$\bso(F) \cap \bta(F)$.
Thus, Condition~\eqref{it:globularcond3} holds and the proof is complete.
\end{proof}

\SS \label{ss:iterative-source-target}

\remark
The same properties which allowed us to show the globular identities in the proof of~\cref{thm:gobular-structure} show that input and output boundaries can be computed iteratively.
Using \cref{s:computing_sk_and_tk} and \cref{s:subdivision} we compute that
$$\bso_k(F) = \bso(\pi_{k+1}(F)) = \bso(\pi_{k+1}(\bso(F))) = \bso(\bso(\pi_{k+2}(F))) = \cdots = \bso(\bso(\cdots \bso(F))).$$
Therefore, the orientation structure of a framed polytope is completely determined by its source and target sets.

\SS

The face lattice $\faces$ of a framed polytope is an instance of an \defn{oriented graded poset}, that is a graded poset together with an edge labelling of its Hasse diagram by $\{-,+\}$.

\SS

\remark
The augmented chain complex from~\cref{d:associated_chain_complex} can be defined for any oriented graded poset which is \emph{oriented thin}~\cite[Par.~11.1.6]{Hadzihasanovic24}.
Moreover, the former satisfies~\cref{ss:atoms} and~\cref{t:unital} whenever the latter is a regular directed complex, see \cite[Lem.~11.2.9 \& Prop.~11.2.11]{Hadzihasanovic24}.
As we have seen in~\cref{p:oriented-thin} and~\cref{thm:gobular-structure}, framed polytopes satisfy both of these conditions; we can thus recover the above two results as particular instances of the general theory developed in~\cite{Hadzihasanovic24}.

\SS

Much in the same way as molecules were defined for a polytope in~\cref{def:atoms-molecules}, one can define molecules more generally as a class of oriented graded posets~\cite[Def.~3.3.2]{Hadzihasanovic24}.

\SS

\theorem (\cite[Thm.~5.2.12]{Hadzihasanovic24})
Any oriented graded poset $P$ has an associated $\omega$-category $\Mol_{/P}$, whose
\begin{itemize}
	\item $d$-cells are the isomorphism classes of oriented graded poset morphisms $f: U \to P$ where the source is an $k$-dimensional molecule with $k \leq d$,
	\item identities are given by inclusions,
	\item $k$-compositions are given for pairs of morphisms $f:U \to P$, $g \colon V \to P$, where $U,V$ are $k$-composable molecules, by the isomorphism class of the morphism $f \circ_k g \colon U \circ_k V \to P$.
\end{itemize}

\begin{remark}
	This $\omega$-category is similar, but distinct from the \emph{partial} $\omega$-category of \cite[Prop.~1.23]{Hadzihasanovic20} and \cite[Prop.~2.9]{Steiner93}.
\end{remark}

\SS \label{prop:chain-implications}

One has 4 notions of acyclicity for $\Mol_{/P}$, it can be acyclic, strongly dimension-wise acyclic, dimension-wise acyclic, and frame-acyclic.
They are related by the following chain of strict implications \cite[Ch.~8]{Hadzihasanovic24}
\[ \text{acyclic} \implies \text{strongly dim-wise acyclic} \implies \text{dim-wise acyclic} \implies \text{frame-acyclic}.\]

\SS \label{thm:freeness-molecules}

\theorem (\cite[Cor.~5.3.10,Thm.~8.2.14,Prop.~8.3.23]{Hadzihasanovic24})
Let $P$ be an oriented graded poset.
\begin{itemize}
	\item If $P$ is a regular directed complex, then the $\omega$-category $\Mol_{/P}$ is generated by the atoms of~$P$.
	\item If $P$ is frame-acyclic, then the $\omega$-category $\Mol_{/P}$ is free on the atoms of $P$, that is, $\Mol_{/P}$ is a polygraph.
	\item If $P$ is strongly dimension-wise acyclic, then every oriented graded poset morphism $U \to P$ from a molecule $U$ to $P$ is injective.
\end{itemize}

\SS

Given a regular directed complex $P$, one can also take cellular chains $\chains(P)$, and apply Steiner's $\nu$ functor, obtaining another $\omega$-category $\nu(\chains(P))$.

\SS \label{thm:comparison-molecules-chains}

\begin{samepage}
\theorem (\cite[Prop.~11.2.17,Thm.~11.2.18,Prop.~11.2.35]{Hadzihasanovic24})
If $P$ is dimension-wise acyclic, then we have an isomorphism of $\omega$-categories
\[ \Mol_{/P} \cong \nu(\chains(P)).\]
Moreover, we have that
\begin{itemize}
	\item $\Mol_{/P}$ is acyclic $\iff \nu(\chains(P))$ is strongly loop-free,
	\item $\Mol_{/P}$ is dimension-wise acyclic $\iff \nu(\chains(P))$ is loop-free.
\end{itemize}
\end{samepage}

\SS

\cref{t:comparison-omega-cats} summarizes this correspondence, and compares with notions of acyclicity for the partial $\omega$-category of molecules $M(P)$ considered in \cite{Steiner93,Hadzihasanovic20}.

\begin{table}[h!]
	\begin{center}
	\begin{tabular}{c|c|c}
	$M(P)$ & $\Mol_{/P}$ & $\nu(\chains(P))$ \\
	\hline
	totally loop-free & acyclic & strongly loop-free \\
	loop-free & strongly dimension-wise acyclic & - \\
	- & dimension-wise acyclic & loop-free \\
	split & frame-acyclic & -
	\end{tabular}
	\end{center}
	\bigskip
	\caption{Comparison of the acyclicity criteria for the partial $\omega$-category $M(P)$ \cite{Steiner93} and the $\omega$-categories $\Mol_{/P}$ \cite{Hadzihasanovic24} and $\nu(\chains(P))$ \cite{steiner2004omega} associated to a regular directed complex $P$.}
	\label{t:comparison-omega-cats}
\end{table}

\SS

It would be interesting to know if the strict chain of implications \cref{prop:chain-implications} holds for framed polytopes.
In particular, it seems desirable to determine if all framed polytopes are frame-acyclic, and thus always define polygraphs.
It would also be interesting to compare $\Mol_{/\faces}$ and $\nu(\chains(P))$ in the non loop-free case.



==> sec/operations.tex <==
% !TEX root = ../polycat.tex

\subsection{Operations on framed polytopes}


\subsubsection{}

\theorem
	The product $P \times Q$ of two framed polytopes $P,Q$ is a framed polytope.
	Moreover, if both $P$ and $Q$ are loop-free, then so is $P \times Q$.





==> sec/pasting.tex <==
% !TEX root = ../fib_poly.tex

\tikzstyle{object} = [circle, fill, minimum size=2pt, inner sep=0pt, outer sep=0pt]

\begin{tikzpicture}[auto, node distance=2cm,>=latex']
	\node[object] (0) {};
	\node[object] (1) at (1,1) {};
	\node[object] (2) at (3,1) {};
	\node[object] (3) at (4,0) {};
	\node[object] (4) at (5,0) {};
	\node[object] (5) at (6.5,0) {};
	\node[object] (6) at (8,1) {};
	\node[object] (7) at (9,0) {};

	\draw[->]
	(0) edge (1)
	(1) edge (2)
	(2) edge (3)
	(3) edge (4);

	\draw[->] (4) to[out=90,in=90] (5);
	\draw[->] (4) to[out=-90,in=-90] (5);

	\draw[->]
	(5) edge (6)
	(6) edge (7)
	(5) edge (7);

	\node[object] (21) at (1,-1) {};
	\node[object] (22) at (3,-1) {};

	\draw[->]
	(0) edge (21)
	(21) edge (22)
	(22) edge (3);

	\node[object] (8) at (2,0) {};
	\draw[->]
	(0) edge (8)
	(8) edge (2)
	(8) edge (22);

	\node at (1.5,.5){$\Downarrow$};
	\node at (1.5,-.5){$\Downarrow$};
	\node at (3,0){$\Downarrow$};
	\node at (5.8,0){$\Downarrow$};
	\node at (8,.4){$\Downarrow$};
\end{tikzpicture}
